Practical Differentially Private Top-$k$ Selection with Pay-what-you-get Composition

We study the problem of top-$k$ selection over a large domain universe subject to user-level differential privacy. Typically, the exponential mechanism or report noisy max are the algorithms used to solve this problem. However, these algorithms require querying the database for the count of each domain element. We focus on the setting where the data domain is unknown, which is different than the setting of frequent itemsets where an apriori type algorithm can help prune the space of domain elements to query. We design algorithms that ensures (approximate) $(\epsilon,\delta>0)$-differential privacy and only needs access to the true top-$\bar{k}$ elements from the data for any chosen $\bar{k} \geq k$. This is a highly desirable feature for making differential privacy practical, since the algorithms require no knowledge of the domain. We consider both the setting where a user's data can modify an arbitrary number of counts by at most 1, i.e. unrestricted sensitivity, and the setting where a user's data can modify at most some small, fixed number of counts by at most 1, i.e. restricted sensitivity. Additionally, we provide a pay-what-you-get privacy composition bound for our algorithms. That is, our algorithms might return fewer than $k$ elements when the top-$k$ elements are queried, but the overall privacy budget only decreases by the size of the outcome set.

==> challenges.tex <==
% !TEX root = main.tex

\subsection{Challenges for Privacy in Existing Systems}

%Suppose a company has existing infrastructure to run quick, real-time data analytics on large datasets.  To design differentially private algorithms that are built on top of this existing system, we need to consider how the original data is preprocessed for efficiency and how that might affect the more upstream differentially private algorithms we design.  For example, consider a system that computes the top-$k$ most frequent elements that distinct users have contributed to.  To make things efficient, the system will distribute the elements from distinct users over a large dataset to multiple servers.  Each server will then compute the top-$\bk$ most frequent elements for $\bk \geq k$ and report this to an aggregator, which only has access to these distributed top-$\bk$ histograms.  The aggregator then computes the top-$k$ elements on the aggregated data and returns this to the data analyst.  
%
%The challenge to designing a differentially private algorithm at the aggregator level is that if one user's data were removed from the original dataset, then that might cause one or many elements to not be part of the top-$\bk$ on a server, thus causing the aggregator to never see those elements.  Even if the data domain is known, the count of one element might go from roughly (assuming number of servers and $\bk$ is constant) $n$, where $n$ is the total number of records, to zero.  Hence, a na\"ive approach to ensure differential privacy would be to add noise to each count that would scale with $n$.  Alternatively, to avoid the preprocessing, we could simply have each server return all the data, i.e. $\bk$ becomes $d$, and then add noise to the full histogram.  However this might come at the cost of losing efficiency.  Designing differentially private algorithms get even more difficult when the domain of elements is not known. In this work, we present a way to balance the efficiency of an existing system and privacy, with tuning knobs $\bk$ and $\diffp$, respectively. 
%
%Implementing differential privacy in an efficient way is a common issue in existing data processing infrastructure, such as online analytical processing (OLAP) systems.  In particular, for columnar data structures, a query only accesses the attributes necessary to answer it, rather than scanning each row of a data table and discarding any unnecessary information.  For example, if we want to restrict the sensitivity of a query, we would want to access not just the attributes necessary to answer the query, but also the user labels corresponding to the entries that are in a separate column of data.  Modifying the raw data to restrict sensitivity of some queries would create a bottleneck in data processing and would affect several other queries that access that same data.  In order to make differential privacy more practical, one would hope to leverage the efficient systems that are already in place, carefully considering each computation being done on the data.   


Suppose a company has existing infrastructure to run quick, real-time data analytics on large datasets containing many dimensions of user data distributed across multiple servers. In theory, sorting across one of these dimensions to return the sorted list is a solved problem taking $n \log(n)$ time, but for massive datasets this is too computationally expensive for real-time analytics, particularly in communicating the list of size $n$ across servers. In addition, we often want to aggregate user data across each dimension and return the top-$k$ dimensions after this aggregation, requiring further computation. On top of this, the dimensions often correspond to all possible user actions, which is often massive and sometimes even unknown. It can then be both inefficient and impossible to store one users data as a single row, and each users data will be distributed in columnar data structures across many servers. 


Constructing data processing infrastructure to compute top-$k$ queries on these massive datasets, such as online analytical processing (OLAP) systems, is one of the most fundamental problems in data science. 
Existing data structures for efficiently solving this problem are often quite involved, and will particularly be able to achieve speedups by minimizing both the amount of scanned input data and the amount of data communicated across servers. 
These restrictions make differential privacy particularly difficult.
We could attempt to redesign these data processing techniques in a differentially private manner while still maintaining a sufficient level of efficiency, or instead design differentially private algorithms that are built on top of this existing system. To achieve the latter, we assume that we can never access the entire sorted list, and will always be restricted to only accessing the top-$\bk$ for some $\bk << d$.
 
 
 
 


%With such a system in place, it is desirable to leverage the low latency data analytics system to then also provide differentially private results.  However, some preprocessing on the data that was used to make analytics more efficient makes it difficult for including some off the shelf differentially private algorithms.  For example, it might be impossible to limit how many counts on different domain elements a user can impact, thus preventing us from bounding sensitivity, which is crucial in some differentially private algorithms.  However, our aim is to still provide user-level privacy guarantees, where an entire user's data can be removed and the outcomes will be close to the outcomes with that user's data included.  To our knowledge, no other work studies the problem of top-$k$ selection under the restriction of not knowing the data domain or at least knowing some structure on the domain, e.g. frequent itemsets.  Since top-$k$ queries are usually part of an exploratory analysis, we want to assume the analyst has no knowledge \emph{a priori} about the domain.


%We envision that there is an existing system, designed to take the raw data and distribute it across several, perhaps hundreds, of servers that cannot communicate with one another.  Then there is a broker that aggregates the results from these servers to provide fast, real-time analytics.  To enable efficient analytics, some preprocessing on the data has occurred.  This preprocessing can impact the sensitivity of the later analyses arbitrarily.  

%For example, imagine that a query is asked for the top-$k$ webpages that were viewed by distinct users.  The broker then asks each server to provide its top-$10k$ webpages that were viewed by distinct users along with their counts, or $H_{10k}(\bbx)$, and with these results the broker aggregates them together and sorts to obtain the top-$k$.  To obtain the distinct elements in the count-distinct problem in a highly efficient way on the servers and the broker, we can use the HyperLogLog algorithm \cite{DurandFl03}. Note that this will provide an estimate to the top-$k$, but assuming the distribution of data across the servers is pretty uniform, this will give accurate results.  If we were to incorporate differential privacy after the preprocessing has occurred, there is a major issue because when one person's data is deleted, even if it is a single webpage, it might cause the webpage on a server to not be included in its top-$10k$, effectively dropping its count to zero. If the domain were known (which we will not assume in this work) and we assume each user can visit at most one webpage, a naive approach to incorporating differential privacy would be to add noise to each count.  However, the noise would have to scale with the sensitivity, i.e. the amount one user can alter the counts, which can be very large since one user can drop a count from the $10k^{(\text{th})}$ highest value on a server to zero.  Hence, preprocessing on the data can cause the differential privacy parameters to grow.  

%An additional challenge is that the users can modify an arbitrary number of domain elements.  We can ensure that a user cannot impact the count of a particular domain element by at most one using count-distinct, but it is very inefficient to limit the number of distinct elements a user can alter to some fixed upper bound.  Ideally, we would like to not alter the dataset and maintain the low-latency infrastructure in the design of our differentially private algorithms.  
